Scaling Up Reachability Analysis for Rectangular Automata with Random Clocks

This paper presents optimizations to improve the scalability of reachability analysis on a subclass of hybrid automata extended with stochasticity. The optimizations target different components of the analysis, such as quantifier elimination for state set projection, and automated parameter selection during the numerical integration. Most importantly, whereas the original method combines forward and backward reachability, we show that the usage of backward reachability is optional for computing maximal reachability probabilities.

==> plots/car_1det_abc_sing_rect_extract_combined.tex <==
\pgfplotstableread[col sep=comma]{csv/results_br_car_plot.csv}\datatable

\begin{tikzpicture}[baseline=(current bounding box.north),font=\sffamily, fill opacity = 0.75, opacity = 0.75]
    \begin{axis}[colormap/viridis,
    scale only axis=true,
    title=\ccar ABC,
    title style={yshift=-0.2cm},
        ybar stacked,
        ylabel={Comp. time in \si{\second}}, 
        xticklabels={$\polyfb$,$\polyfwd$,$\polyfb$,$\polyfwd$},
        xtick=data,
        minor x tick num=1,
        enlarge x limits=0.1,
        legend pos=north west,
        grid style=dashed,
        bar width=0.1cm,
        ymin=0,        
        width=1.9cm,
        height=0.2\textwidth,
        legend style={
      font=\footnotesize,
      cells={anchor=west},
      legend columns=2,
      at={(0.3,-0.20)},
      anchor=north,
      /tikz/every even column/.append style={column sep=0.2cm}
    },
     draw group line={rectangular}{0}{\text{S}}{-0.5cm}{1pt},    
     draw group line={rectangular}{1}{\text{R}}{-0.5cm}{1pt},
    ]
    

    \addplot+[color=color-time-forward, fill, thick, name path=A] table[x=table_index, y=t_flowpipe, col sep=comma] \datatable;
    \addplot+[color=color-time-stochastic-processing, fill, thick, name path=A] table[x=table_index, y=t_stochastic_processing, col sep=comma] \datatable;
    \addplot+[color=color-time-refinement-preprocessing, fill, thick, name path=A] table[x=table_index, y=t_refinement_preprocessing, col sep=comma] \datatable;
    \addplot+[color=color-time-refinement, fill, thick, name path=A] table[x=table_index, y=t_refinement, col sep=comma] \datatable;
     \addplot+[color=color-time-integration, fill, thick, name path=A] table[x=table_index, y=t_integration, col sep=comma] \datatable;
    \end{axis}
\end{tikzpicture}

==> plots/ebike_1det_sing_rect_extract_combined.tex <==
\pgfplotstableread[col sep=comma]{csv/results_br_ebike_plot.csv}\datatable
\begin{tikzpicture}[baseline=(current bounding box.north),font=\sffamily, fill opacity = 0.75, opacity = 0.75]
    \begin{axis}[colormap/viridis,
    scale only axis=true,
    title=\cebike,
        title style={yshift=-0.2cm},
        ybar stacked,
        xticklabels={$\polyfb$,$\polyfwd$,$\polyfb$,$\polyfwd$},
        xtick=data,
        minor x tick num=1,
        enlarge x limits=0.1,
        legend pos=north west,
        grid style=dashed,
        bar width=0.1cm,
        ymin=0,        
        width=1.9cm,
        height=0.2\textwidth,
        legend style={
      font=\footnotesize,
      cells={anchor=west},
      legend columns=2,
      at={(0.3,-0.20)},
      anchor=north,
      /tikz/every even column/.append style={column sep=0.2cm}
    },
    legend to name=named,
     draw group line={rectangular}{0}{\text{S}}{-0.5cm}{1pt},    
     draw group line={rectangular}{1}{\text{R}}{-0.5cm}{1pt},
    ]
    

    \addplot+[color=color-time-forward, fill, thick, name path=A] table[x=table_index, y=t_flowpipe, col sep=comma] \datatable;   
    \addplot+[color=color-time-stochastic-processing, fill, thick, name path=A] table[x=table_index, y=t_stochastic_processing, col sep=comma] \datatable;
    \addplot+[color=color-time-refinement-preprocessing, fill, thick, name path=A] table[x=table_index, y=t_refinement_preprocessing, col sep=comma] \datatable;
    \addplot+[color=color-time-refinement, fill, thick, name path=A] table[x=table_index, y=t_refinement, col sep=comma] \datatable;
    \addplot+[color=color-time-integration, fill, thick, name path=A] table[x=table_index, y=t_integration, col sep=comma] \datatable;     
    \legend{Reachability, Stochastic proc., Refinement preproc., Refinement, Integration}
    \end{axis}
\end{tikzpicture}

==> tikzsettings.tex <==
\makeatletter
\newcounter{groupcount}
\pgfplotsset{
    draw group line/.style n args={5}{
        after end axis/.append code={
            \setcounter{groupcount}{0}
            \pgfplotstableforeachcolumnelement{#1}\of\datatable\as\cell{%
                \def\temp{#2}
                \ifx\temp\cell
                    \ifnum\thegroupcount=0
                        \stepcounter{groupcount}
                        \pgfplotstablegetelem{\pgfplotstablerow}{[index]0}\of\datatable
                        \coordinate [yshift=#4] (startgroup) at (axis cs:\pgfplotsretval,0);
                    \else
                        \stepcounter{groupcount}
                        \pgfplotstablegetelem{\pgfplotstablerow}{[index]0}\of\datatable
                        \coordinate [yshift=#4] (endgroup) at (axis cs:\pgfplotsretval,0);
                    \fi
                \else
                    \ifnum\thegroupcount>1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=north] {#3} (endgroup);
                    \fi
                \fi
            }
            \ifnum\thegroupcount>1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=north] {#3} (endgroup);
            \fi
            \ifnum\thegroupcount=1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] ($(startgroup)-(1.5mm,0)$) -- node [anchor=north] {#3} ($(startgroup)+(1.5mm,0)$);
            \fi
        }
    }
}
\makeatother

\pgfplotsset{
tick label style={font=\footnotesize},
label style={font=\small},
legend style={font=\footnotesize},
}

\pgfmathdeclarefunction{gauss}{3}{%
	\pgfmathparse{1/(#3*sqrt(2*pi))*exp(-((#1-#2)^2)/(2*#3^2))}%
}

\pgfmathdeclarefunction{uniformPDF}{2}{%
	\pgfmathparse{1/(#2-#1}%
}

\pgfmathdeclarefunction{expPDF}{2}{%
	\pgfmathparse{#2 * exp(-#2 * #1)}%
}

\pgfmathdeclarefunction{nullPDF}{2}{%
	\pgfmathparse{#2-#2}%
}

\tikzstyle{refinement}=[pattern=north west lines, pattern color = goaltrace1] %
\tikzstyle{refinement2}=[pattern=north east lines, pattern color = goaltrace2] %

\tikzstyle{mycrosshatching}=[pattern=north west lines, pattern color = gray] %

